Kron-based Model-order Reduction of Open Mass-action Kinetics Chemical Reaction Networks

We propose a Kron-based model-order reduction method for mass-action kinetics chemical reaction networks (CRN) with constant inflow and proportional outflow. The reduced-order models preserve the CRN structure and we establish that the resulting reduced-order models have the same DC-gain or zero-moment as that of the full-order ones. Subsequently, we present the spectrum interlacing property of the Kron-reduced open CRN and propose the use of Gramians-based approach for single-species single-substrate chemical network to get the upper-bound of approximation error and to use it in determining a good set of nodes to be removed systematically. Finally, we evaluate the applicability and efficacy of our results in two well-known biochemical kinetic models: the activated sludge model (ASM) 1 and McKeithan's T-cell receptor model.

==> ka-newcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                 
%%  NEWCOMMANDS                    
%%                                 
%%  version 9  22/01/15           
%%                                 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\col}{col}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\bdiag}{blockdiag}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\inte}{int}
\DeclareMathOperator{\clo}{cl}
\DeclareMathOperator{\rint}{rint}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\graph}{graph}
\DeclareMathOperator{\dis}{dis}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\Imag}{Im}




\let\leq\leqslant
\let\geq\geqslant
\let\emptyset\varnothing

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \calA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \sfA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sfA}{\ensuremath{\mathsf{A}}}
\newcommand{\sfB}{\ensuremath{\mathsf{B}}}
\newcommand{\sfC}{\ensuremath{\mathsf{C}}}
\newcommand{\sfD}{\ensuremath{\mathsf{D}}}
\newcommand{\sfE}{\ensuremath{\mathsf{E}}}
\newcommand{\sfF}{\ensuremath{\mathsf{F}}}
\newcommand{\sfG}{\ensuremath{\mathsf{G}}}
\newcommand{\sfH}{\ensuremath{\mathsf{H}}}
\newcommand{\sfI}{\ensuremath{\mathsf{I}}}
\newcommand{\sfJ}{\ensuremath{\mathsf{J}}}
\newcommand{\sfK}{\ensuremath{\mathsf{K}}}
\newcommand{\sfL}{\ensuremath{\mathsf{L}}}
\newcommand{\sfM}{\ensuremath{\mathsf{M}}}
\newcommand{\sfN}{\ensuremath{\mathsf{N}}}
\newcommand{\sfO}{\ensuremath{\mathsf{O}}}
\newcommand{\sfP}{\ensuremath{\mathsf{P}}}
\newcommand{\sfQ}{\ensuremath{\mathsf{Q}}}
\newcommand{\sfR}{\ensuremath{\mathsf{R}}}
\newcommand{\sfS}{\ensuremath{\mathsf{S}}}
\newcommand{\sfT}{\ensuremath{\mathsf{T}}}
\newcommand{\sfU}{\ensuremath{\mathsf{U}}}
\newcommand{\sfV}{\ensuremath{\mathsf{V}}}
\newcommand{\sfW}{\ensuremath{\mathsf{W}}}
\newcommand{\sfX}{\ensuremath{\mathsf{X}}}
\newcommand{\sfY}{\ensuremath{\mathsf{Y}}}
\newcommand{\sfZ}{\ensuremath{\mathsf{Z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \hata
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hata}{\ensuremath{\hat{a}}}
\newcommand{\hatb}{\ensuremath{\hat{b}}}
\newcommand{\hatc}{\ensuremath{\hat{c}}}
\newcommand{\hatd}{\ensuremath{\hat{d}}}
\newcommand{\hate}{\ensuremath{\hat{e}}}
\newcommand{\hatf}{\ensuremath{\hat{f}}}
\newcommand{\hatg}{\ensuremath{\hat{g}}}
\newcommand{\hath}{\ensuremath{\hat{h}}}
\newcommand{\hati}{\ensuremath{\hat{i}}}
\newcommand{\hatj}{\ensuremath{\hat{j}}}
\newcommand{\hatk}{\ensuremath{\hat{k}}}
\newcommand{\hatl}{\ensuremath{\hat{l}}}
\newcommand{\hatm}{\ensuremath{\hat{m}}}
\newcommand{\hatn}{\ensuremath{\hat{n}}}
\newcommand{\hato}{\ensuremath{\hat{o}}}
\newcommand{\hatp}{\ensuremath{\hat{p}}}
\newcommand{\hatq}{\ensuremath{\hat{q}}}
\newcommand{\hatr}{\ensuremath{\hat{r}}}
\newcommand{\hats}{\ensuremath{\hat{s}}}
\newcommand{\hatt}{\ensuremath{\hat{t}}}
\newcommand{\hatu}{\ensuremath{\hat{u}}}
\newcommand{\hatv}{\ensuremath{\hat{v}}}
\newcommand{\hatw}{\ensuremath{\hat{w}}}
\newcommand{\hatx}{\ensuremath{\hat{x}}}
\newcommand{\haty}{\ensuremath{\hat{y}}}
\newcommand{\hatz}{\ensuremath{\hat{z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \hatA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hatA}{\ensuremath{\hat{A}}}
\newcommand{\hatB}{\ensuremath{\hat{B}}}
\newcommand{\hatC}{\ensuremath{\hat{C}}}
\newcommand{\hatD}{\ensuremath{\hat{D}}}
\newcommand{\hatE}{\ensuremath{\hat{E}}}
\newcommand{\hatF}{\ensuremath{\hat{F}}}
\newcommand{\hatG}{\ensuremath{\hat{G}}}
\newcommand{\hatH}{\ensuremath{\hat{H}}}
\newcommand{\hatI}{\ensuremath{\hat{I}}}
\newcommand{\hatJ}{\ensuremath{\hat{J}}}
\newcommand{\hatK}{\ensuremath{\hat{K}}}
\newcommand{\hatL}{\ensuremath{\hat{L}}}
\newcommand{\hatM}{\ensuremath{\hat{M}}}
\newcommand{\hatN}{\ensuremath{\hat{N}}}
\newcommand{\hatO}{\ensuremath{\hat{O}}}
\newcommand{\hatP}{\ensuremath{\hat{P}}}
\newcommand{\hatQ}{\ensuremath{\hat{Q}}}
\newcommand{\hatR}{\ensuremath{\hat{R}}}
\newcommand{\hatS}{\ensuremath{\hat{S}}}
\newcommand{\hatT}{\ensuremath{\hat{T}}}
\newcommand{\hatU}{\ensuremath{\hat{U}}}
\newcommand{\hatV}{\ensuremath{\hat{V}}}
\newcommand{\hatW}{\ensuremath{\hat{W}}}
\newcommand{\hatX}{\ensuremath{\hat{X}}}
\newcommand{\hatY}{\ensuremath{\hat{Y}}}
\newcommand{\hatZ}{\ensuremath{\hat{Z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \bara
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bara}{\ensuremath{\bar{a}}}
\newcommand{\barb}{\ensuremath{\bar{b}}}
\newcommand{\barc}{\ensuremath{\bar{c}}}
\newcommand{\bard}{\ensuremath{\bar{d}}}
\newcommand{\bare}{\ensuremath{\bar{e}}}
\newcommand{\barf}{\ensuremath{\bar{f}}}
\newcommand{\barg}{\ensuremath{\bar{g}}}
\newcommand{\barh}{\ensuremath{\bar{h}}}
\newcommand{\bari}{\ensuremath{\bar{i}}}
\newcommand{\barj}{\ensuremath{\bar{j}}}
\newcommand{\bark}{\ensuremath{\bar{k}}}
\newcommand{\barl}{\ensuremath{\bar{l}}}
\newcommand{\barm}{\ensuremath{\bar{m}}}
\newcommand{\barn}{\ensuremath{\bar{n}}}
\newcommand{\baro}{\ensuremath{\bar{o}}}
\newcommand{\barp}{\ensuremath{\bar{p}}}
\newcommand{\barq}{\ensuremath{\bar{q}}}
\newcommand{\barr}{\ensuremath{\bar{r}}}
\newcommand{\bars}{\ensuremath{\bar{s}}}
\newcommand{\bart}{\ensuremath{\bar{t}}}
\newcommand{\baru}{\ensuremath{\bar{u}}}
\newcommand{\barv}{\ensuremath{\bar{v}}}
\newcommand{\barw}{\ensuremath{\bar{w}}}
\newcommand{\barx}{\ensuremath{\bar{x}}}
\newcommand{\bary}{\ensuremath{\bar{y}}}
\newcommand{\barz}{\ensuremath{\bar{z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \barA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\barA}{\ensuremath{\bar{A}}}
\newcommand{\barB}{\ensuremath{\bar{B}}}
\newcommand{\barC}{\ensuremath{\bar{C}}}
\newcommand{\barD}{\ensuremath{\bar{D}}}
\newcommand{\barE}{\ensuremath{\bar{E}}}
\newcommand{\barF}{\ensuremath{\bar{F}}}
\newcommand{\barG}{\ensuremath{\bar{G}}}
\newcommand{\barH}{\ensuremath{\bar{H}}}
\newcommand{\barI}{\ensuremath{\bar{I}}}
\newcommand{\barJ}{\ensuremath{\bar{J}}}
\newcommand{\barK}{\ensuremath{\bar{K}}}
\newcommand{\barL}{\ensuremath{\bar{L}}}
\newcommand{\barM}{\ensuremath{\bar{M}}}
\newcommand{\barN}{\ensuremath{\bar{N}}}
\newcommand{\barO}{\ensuremath{\bar{O}}}
\newcommand{\barP}{\ensuremath{\bar{P}}}
\newcommand{\barQ}{\ensuremath{\bar{Q}}}
\newcommand{\barR}{\ensuremath{\bar{R}}}
\newcommand{\barS}{\ensuremath{\bar{S}}}
\newcommand{\barT}{\ensuremath{\bar{T}}}
\newcommand{\barU}{\ensuremath{\bar{U}}}
\newcommand{\barV}{\ensuremath{\bar{V}}}
\newcommand{\barW}{\ensuremath{\bar{W}}}
\newcommand{\barX}{\ensuremath{\bar{X}}}
\newcommand{\barY}{\ensuremath{\bar{Y}}}
\newcommand{\barZ}{\ensuremath{\bar{Z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \bbA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbA}{\ensuremath{\mathbb{A}}}
\newcommand{\bbB}{\ensuremath{\mathbb{B}}}
\newcommand{\bbC}{\ensuremath{\mathbb{C}}}
\newcommand{\bbD}{\ensuremath{\mathbb{D}}}
\newcommand{\bbE}{\ensuremath{\mathbb{E}}}
\newcommand{\bbF}{\ensuremath{\mathbb{F}}}
\newcommand{\bbG}{\ensuremath{\mathbb{G}}}
\newcommand{\bbH}{\ensuremath{\mathbb{H}}}
\newcommand{\bbI}{\ensuremath{\mathbb{I}}}
\newcommand{\bbJ}{\ensuremath{\mathbb{J}}}
\newcommand{\bbK}{\ensuremath{\mathbb{K}}}
\newcommand{\bbL}{\ensuremath{\mathbb{L}}}
\newcommand{\bbM}{\ensuremath{\mathbb{M}}}
\newcommand{\bbN}{\ensuremath{\mathbb{N}}}
\newcommand{\bbO}{\ensuremath{\mathbb{O}}}
\newcommand{\bbP}{\ensuremath{\mathbb{P}}}
\newcommand{\bbQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\bbR}{\ensuremath{\mathbb{R}}}
\newcommand{\bbS}{\ensuremath{\mathbb{S}}}
\newcommand{\bbT}{\ensuremath{\mathbb{T}}}
\newcommand{\bbU}{\ensuremath{\mathbb{U}}}
\newcommand{\bbV}{\ensuremath{\mathbb{V}}}
\newcommand{\bbW}{\ensuremath{\mathbb{W}}}
\newcommand{\bbX}{\ensuremath{\mathbb{X}}}
\newcommand{\bbY}{\ensuremath{\mathbb{Y}}}
\newcommand{\bbZ}{\ensuremath{\mathbb{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \tta
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tta}{{\tt a}}
\newcommand{\ttb}{{\tt b}}
\newcommand{\ttc}{{\tt c}}
\newcommand{\ttd}{{\tt d}}
\newcommand{\tte}{{\tt e}}
\newcommand{\ttf}{{\tt f}}
\newcommand{\ttg}{{\tt g}}
\newcommand{\tth}{{\tt h}}
\newcommand{\tti}{{\tt i}}
\newcommand{\ttj}{{\tt j}}
\newcommand{\ttk}{{\tt k}}
\newcommand{\ttl}{{\tt l}}
\newcommand{\ttm}{{\tt m}}
\newcommand{\ttn}{{\tt n}}
\newcommand{\tto}{{\tt o}}
\newcommand{\ttp}{{\tt p}}
\newcommand{\ttq}{{\tt q}}
\newcommand{\ttr}{{\tt r}}
\newcommand{\tts}{{\tt s}}
\newcommand{\ttt}{{\tt t}}
\newcommand{\ttu}{{\tt u}}
\newcommand{\ttv}{{\tt v}}
\newcommand{\ttw}{{\tt w}}
\newcommand{\ttx}{{\tt x}}
\newcommand{\tty}{{\tt y}}
\newcommand{\ttz}{{\tt z}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bmat}{\begin{matrix}}
\newcommand{\emat}{\end{matrix}}
\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}
\newcommand{\bbma}{\begin{bmatrix*}[r]}
\newcommand{\ebma}{\end{bmatrix*}}
\newcommand{\bpm}{\begin{pmatrix}}
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\bvm}{\begin{vmatrix}}
\newcommand{\evm}{\end{vmatrix}}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ben}{\renewcommand{\labelenumi}{\arabic{enumi}.}
\renewcommand{\theenumi}{\arabic{enumi}}\begin{enumerate}}

\newcommand{\een}{\end{enumerate}}

\newcommand{\beni}{\renewcommand{\labelenumi}{\roman{enumi}.}
\renewcommand{\theenumi}{\roman{enumi}}\begin{enumerate}}

\newcommand{\eeni}{\end{enumerate}}

\newcommand{\bena}{\renewcommand{\labelenumi}{\alph{enumi}.}
\renewcommand{\theenumi}{\alph{enumi}}\begin{enumerate}}

\newcommand{\eena}{\end{enumerate}}

\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\bthe}{\begin{theorem}}
\newcommand{\ethe}{\end{theorem}}
\newcommand{\blem}{\begin{lemma}}
\newcommand{\elem}{\end{lemma}}
\newcommand{\bprop}{\begin{proposition}}
\newcommand{\eprop}{\end{proposition}}
\newcommand{\bex}{\begin{example}}
\newcommand{\eex}{\end{example}}
\newcommand{\bas}{\begin{assumption}}
\newcommand{\eas}{\end{assumption}}
\newcommand{\bre}{\begin{remark}}
\newcommand{\ere}{\end{remark}}
\newcommand{\bcor}{\begin{corollary}}
\newcommand{\ecor}{\end{corollary}}
\newcommand{\bdfn}{\begin{definition}}
\newcommand{\edfn}{\end{definition}}
\newcommand{\bcon}{\begin{conjecture}}
\newcommand{\econ}{\end{conjecture}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  NEW OPERATORS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  SHORTHAND MATH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ones}{\ensuremath{1\!\!1}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\half}{\ensuremath{\frac{1}{2}}}
\newcommand{\inv}{\ensuremath{^{-1}}}
\newcommand{\pset}[1]{\ensuremath{\{#1\}}}
\newcommand{\nset}[1]{\ensuremath{\{1,2,\ldots,#1\}}}
\newcommand{\zset}{\ensuremath{\pset{0}}}
\newcommand{\lexleq}{\ensuremath{\preccurlyeq}}
\newcommand{\lexgeq}{\ensuremath{\succcurlyeq}}
\newcommand{\set}[2]{\ensuremath{\left\{#1: #2\right\}}}
\newcommand{\res}[2]{\ensuremath{#1|_{#2}}}
\newcommand{\abs}[1]{\ensuremath{| #1 |}}
\newcommand{\norm}[1]{\ensuremath{\| #1 \|}}
\newcommand{\inn}[2]{\ensuremath{\langle #1 , #2 \rangle}}
\newcommand{\polar}[1]{\ensuremath{{#1}^\circ}}
\newcommand{\dual}[1]{\ensuremath{{#1}^*}}
\newcommand{\barrier}[1]{\ensuremath{{#1}^{\mathrm{b}}}}
\newcommand{\rec}[1]{\ensuremath{{#1}^{\infty}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  SETS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{\ensuremath{\mathbb R}}
\newcommand{\C}{\ensuremath{\mathbb C}}
\newcommand{\N}{\ensuremath{\mathbb N}}
\newcommand{\Z}{\ensuremath{\mathbb Z}}
\newcommand{\Lone}{\ensuremath{L_1}}
\newcommand{\Loneloc}{\ensuremath{L_{1,\mathrm{loc}}}}
\newcommand{\Ltwo}{\ensuremath{L_2}}
\newcommand{\Ltwoloc}{\ensuremath{L_{2,\mathrm{loc}}}}
\newcommand{\Linf}{\ensuremath{L_\infty}}
\newcommand{\Linfloc}{\ensuremath{L_{\infty,\mathrm{loc}}}}
\newcommand{\Cinf}{\ensuremath{C^\infty}}
\newcommand{\Absc}{\ensuremath{\mathrm{AC}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  GEOMETRIC CONTROL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\br}[2]{\ensuremath{\langle #1 \mid \im #2 \rangle}}
\newcommand{\brd}[2]{\ensuremath{\langle \ker #1 \mid #2 \rangle}}
\newcommand{\brn}[2]{\ensuremath{\langle #1 \mid #2 \rangle}}
\newcommand{\calVs}{\ensuremath{\calV^*}}
\newcommand{\calRs}{\ensuremath{\calR^*}}
\newcommand{\calTs}{\ensuremath{\calT^*}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  SYSTEMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\abcd}{\ensuremath{(A,B,C,D)}}
\newcommand{\abcdef}{\ensuremath{(A,B,C,D,E,F)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  MISC
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\BP}{\noindent{\bf Proof. }}
\newcommand{\EP}{\hspace*{\fill} $\blacksquare$\bigskip\noindent}
\newcommand{\qand}{\quad\text{ and }\quad}





